Neutralino Dark Matter in BMSSM Effective Theory

We study thermal neutralino dark matter in an effective field theory extension of the MSSM, called "Beyond the MSSM" (BMSSM) in Dine, Seiberg and Thomas (2007). In this class of effective field theories, the field content of the MSSM is unchanged, but the little hierarchy problem is alleviated by allowing small corrections to the Higgs/higgsino part of the Lagrangian. We perform parameter scans and compute the dark matter relic density. The light Higgsino LSP scenario is modified the most; we find new regions of parameter space compared to the standard MSSM. This involves interesting interplay between the WMAP dark matter bounds and the LEP chargino bound. We also find some changes for gaugino LSPs, partly due to annihilation through a Higgs resonance, and partly due to coannihilation with light stops in models that are ruled in by the new effective terms.

==> references.tex <==
\begin{thebibliography}{99} 

%\cite{Gondolo:2004sc}
\bibitem{Gondolo:2004sc}
  P.~Gondolo, J.~Edsjo, P.~Ullio, L.~Bergstrom, M.~Schelke and E.~A.~Baltz,
  %``DarkSUSY: Computing supersymmetric dark matter properties numerically,''
  JCAP {\bf 0407}, 008 (2004)
  [arXiv:astro-ph/0406204].
  %%CITATION = JCAPA,0407,008;%%

%\cite{Heinemeyer:1998yj}
\bibitem{Heinemeyer:1998yj}
  S.~Heinemeyer, W.~Hollik and G.~Weiglein,
  %``FeynHiggs: a program for the calculation of the masses of the neutral
  %CP-even Higgs bosons in the MSSM,''
  Comput.\ Phys.\ Commun.\  {\bf 124}, 76 (2000)
  [arXiv:hep-ph/9812320].
  %%CITATION = CPHCB,124,76;%%

%\cite{Heinemeyer:1998np}
\bibitem{Heinemeyer:1998np}
  S.~Heinemeyer, W.~Hollik and G.~Weiglein,
  %``The Masses of the neutral CP - even Higgs bosons in the MSSM: Accurate
  %analysis at the two loop level,''
  Eur.\ Phys.\ J.\  C {\bf 9}, 343 (1999)
  [arXiv:hep-ph/9812472].
  %%CITATION = EPHJA,C9,343;%%

%\cite{Degrassi:2002fi}
\bibitem{Degrassi:2002fi}
  G.~Degrassi, S.~Heinemeyer, W.~Hollik, P.~Slavich and G.~Weiglein,
  %``Towards high-precision predictions for the MSSM Higgs sector,''
  Eur.\ Phys.\ J.\  C {\bf 28}, 133 (2003)
  [arXiv:hep-ph/0212020].
  %%CITATION = EPHJA,C28,133;%%

%\cite{Frank:2006yh}
\bibitem{Frank:2006yh}
  M.~Frank, T.~Hahn, S.~Heinemeyer, W.~Hollik, H.~Rzehak and G.~Weiglein,
  %``The Higgs boson masses and mixings of the complex MSSM in the
  %Feynman-diagrammatic approach,''
  JHEP {\bf 0702}, 047 (2007)
  [arXiv:hep-ph/0611326].
  %%CITATION = JHEPA,0702,047;%%

%\cite{Bechtle:2008jh}
\bibitem{Bechtle:2008jh}
  P.~Bechtle, O.~Brein, S.~Heinemeyer, G.~Weiglein and K.~E.~Williams,
  %``HiggsBounds: Confronting Arbitrary Higgs Sectors with Exclusion Bounds from
  %LEP and the Tevatron,''
  arXiv:0811.4169 [hep-ph].
  %%CITATION = ARXIV:0811.4169;%%

\end{thebibliography} 


